Why did the distribution change?

We describe a formal approach based on graphical causal models to identify the "root causes" of the change in the probability distribution of variables. After factorizing the joint distribution into conditional distributions of each variable, given its parents (the "causal mechanisms"), we attribute the change to changes of these causal mechanisms. This attribution analysis accounts for the fact that mechanisms often change independently and sometimes only some of them change. Through simulations, we study the performance of our distribution change attribution method. We then present a real-world case study identifying the drivers of the difference in the income distribution between men and women.

==> preamble.tex <==
\RequirePackage{mathtools}
\RequirePackage{bm}
\RequirePackage{amsmath}

\newcommand{\note}[1]{{\color{red}#1}\xspace}
%\newcommand{\comment}[1]{}

\newcommand{\rvX}{\ensuremath{X}\xspace}
\newcommand{\rvY}{\ensuremath{Y}\xspace}
\newcommand{\rvZ}{\ensuremath{Z}\xspace}
\newcommand{\rvN}{\ensuremath{N}\xspace}
\newcommand{\mrvX}{\ensuremath{\textbf{X}}\xspace}
\newcommand{\PA}{\ensuremath{\mathit{PA}}\xspace}
\newcommand{\pa}{\ensuremath{\mathit{pa}}\xspace}
\newcommand{\dist}{\ensuremath{P}\xspace}
\newcommand{\newdist}{\ensuremath{\tilde{P}}\xspace}
\newcommand{\density}{\ensuremath{p}\xspace}
\newcommand{\entropy}{\ensuremath{H}\xspace}
\newcommand{\shapleyValue}{\ensuremath{\phi}\xspace}

\newcommand{\domainX}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\domainY}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\domainZ}{\ensuremath{\mathcal{Z}}\xspace}

\newcommand{\domainMrvX}{\ensuremath{\bm{\mathcal{X}}}\xspace}

\newcommand{\obsRvX}{\ensuremath{x}\xspace}
\newcommand{\obsRvY}{\ensuremath{y}\xspace}
\newcommand{\obsRvN}{\ensuremath{n}\xspace}
\newcommand{\suppRvX}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\obsMrvX}{\ensuremath{\mathbf{x}}\xspace}

\bmdefine{\mrvZ}{Z}
\bmdefine{\mrvN}{N}
%\bmdefine{\obsMrvX}{x}
\bmdefine{\obsMrvZ}{z}

\newcommand{\causalModel}{\ensuremath{\textswab{C}}\xspace}
\newcommand{\causalGraph}{\ensuremath{G}\xspace}
\newcommand{\causalParameters}{\ensuremath{\Pr}\xspace}

\newcommand{\permutation}{\ensuremath{\sigma}\xspace}
\newcommand{\varianceSymbol}{\ensuremath{\mathrm{Var}}\xspace}
\newcommand{\variance}[1]{\ensuremath{\varianceSymbol\left[#1\right]}\xspace}
\newcommand{\expectationSymbol}{\ensuremath{\mathbb{E}}\xspace}
\newcommand{\expectation}[1]{\ensuremath{\expectationSymbol\left[#1\right]}\xspace}
\newcommand{\expectationWithDist}[2]{\ensuremath{\mathbb{E}_{#1}\left[#2\right]}\xspace}
\newcommand{\exptdist}[2]{\ensuremath{\mathbb{E}_{#1}\left[#2\right]}\xspace}
\newcommand{\doo}{\ensuremath{\mathit{do}}\xspace}
\renewcommand{\Pr}{\ensuremath{P}\xspace}
\newcommand{\FCM}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\shannonEntropy}{\ensuremath{H}\xspace}
\newcommand{\mutualInfo}{\ensuremath{I}\xspace}
%\newcommand{\precedingPlayers}{\ensuremath{\underset{\erelbar{10}}{N}}\xspace}
\newcommand{\precedingPlayers}{\ensuremath{N_{\mathit{prec}}}\xspace}
%\newcommand{\precedingPlayersInclusive}{\ensuremath{\underset{\erelbar{12}}{N}}\xspace}
\newcommand{\precedingPlayersComplement}{\ensuremath{\bar{N}^{\circ}}\xspace}
\newcommand{\precedingPlayersInclusive}{\ensuremath{N^{\bullet}}\xspace}
\newcommand{\precedingPlayersInclusiveComplement}{\ensuremath{\bar{N}^{\bullet}}\xspace}
\newcommand{\marginalContribution}[2]{\ensuremath{C_{#1}\left(#2\right)}\xspace}
\newcommand{\setFunction}{\ensuremath{\nu}\xspace}
\newcommand{\coalition}{\ensuremath{T}\xspace}
\newcommand{\distSummary}{\ensuremath{\psi}\xspace}
\newcommand{\timeIndex}{\ensuremath{A}\xspace}

\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
	#1\;\delimsize|\delimsize|\;#2%
}
\newcommand{\kldSymbol}{\ensuremath{D}\xspace}
\newcommand{\kld}[2]{\ensuremath{\kldSymbol\infdivx{#1}{#2}}\xspace}
\newcommand{\divergenceMeasure}[2]{\ensuremath{d\infdivx{#1}{#2}}\xspace}
\newcommand{\by}[2]{\ensuremath{#1\text{\nobreakdash-by\nobreakdash-}#2}\xspace}
\newcommand{\indep}{\ensuremath{\perp \! \! \! \perp}\xspace}
\newcommand{\dep}{\ensuremath{\not\!\perp\!\!\!\perp}\xspace}

\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}

\newcommand{\scm}{\ensuremath{\textgoth{C}}\xspace}
